Agent Lumos: Unified and Modular Training for Open-Source Language Agents

Closed-source agents suffer from several issues such as a lack of affordability, transparency, and reproducibility, particularly on complex interactive tasks. This motivates the development of open-source alternatives. We introduce LUMOS, one of the first frameworks for training open-source LLM-based agents. LUMOS features a learnable, unified, and modular architecture with a planning module that learns high-level subgoal generation, and a grounding module trained to translate these into actions using various tools in the execution module. The design allows for modular upgrades and wider applicability to diverse interactive tasks. To foster generalizable agent learning, we collect large-scale, unified, and high-quality training annotations derived from diverse ground-truth reasoning rationales across various complex interactive tasks. On 9 datasets, LUMOS exhibits several key advantages: (1) LUMOS excels multiple larger open-source agents on the held-out datasets (unused for training) for each task type. LUMOS even surpasses GPT agents on QA and web tasks; (2) LUMOS outperforms open-source agents produced by chain-of-thoughts and unmodularized integrated training; and (3) LUMOS effectively generalizes to unseen tasks, outperforming 33B-scale agents and domain-specific agents.

==> 2_problem.tex <==
 

==> tab_main.tex <==

% \definecolor{lightgray}{RGB}{233, 233, 233}
% \begin{table}[t]
% \centering
% \caption{A comparative performance analysis between Zero-shot learning (Zero), Few-shot In-Context Learning (ICL), and our proposed Few-shot \lorahub{} learning. In this comparison, we utilize $5$ examples per task as the few-shot demonstrations for both ICL and \lorahub{}. The average (\textit{avg}) performance of \lorahub{} is computed over $5$ distinct runs with different random seeds, while the best (\textit{best}) performance is reported as the maximum value obtained across these runs.
% }
% \label{tab:performance}
% \begin{tabular}{lccc>{\columncolor{lightgray}}c}
% \toprule
% Task & Zero & ICL & \lorahub$_{\rm avg}$ & \lorahub$_{\rm best}$ \\
% \midrule
% Boolean Expressions & 54.0 & \textbf{58.7} & 56.0 & 59.3 \\
% Causal Judgement & 57.5 & 56.3 & \textbf{58.9} & 63.2 \\
% Date Understanding & 15.3 & 22.7 & \textbf{29.6} & 38.0 \\
% Disambiguation & 0.0 & \textbf{69.3} & 46.0 & 69.3 \\
% Dyck Languages & 1.3 & \textbf{7.3} & 0.3 & 1.3 \\
% Formal Fallacies & 51.3 & \textbf{58.0} & 52.1 & 55.3 \\
% Geometric Shapes & 6.7 & \textbf{18.7} & 7.5 & 9.3 \\
% Hyperbaton & 6.7 & \textbf{74.0} & 57.5 & 61.3 \\
% \begin{tabular}[c]{@{}l@{}}Logical Deduction$^\S$ \\ {\small ~~~~~~~~~~~~~(five objects)}\end{tabular} & 21.3 & \textbf{40.0} & 38.1 & 40.7 \\
% \begin{tabular}[c]{@{}l@{}}Logical Deduction$^\S$ \\ {\small ~~~~~~~~~~~~~(seven objects)}\end{tabular} & 12.7 & \textbf{42.0} & 40.3 & 44.7 \\
% \begin{tabular}[c]{@{}l@{}}Logical Deduction$^\S$ \\ {\small ~~~~~~~~~~~~~(three objects)}\end{tabular} & 0.0 & \textbf{51.3} & 49.7 & 51.3 \\
% Movie Recommendation & \textbf{62.7} & 52.7 & 61.1 & 64.0 \\
% Multistep Arithmetic & \textbf{0.7} & \textbf{0.7} & \textbf{0.7} & 0.7 \\
% Navigate & \textbf{47.3} & 44.0 & 46.1 & 49.3 \\
% Object Counting & 34.7 & 32.0 & \textbf{35.0} & 38.0 \\
% Penguins in a Table & 43.5 & 39.1 & \textbf{43.9} & 45.7 \\
% Reasoning about Colored Objects & 32.0 & \textbf{38.7} & 36.5 & 40.7 \\
% Ruin Names & \textbf{23.3} & 18.7 & 21.0 & 23.3 \\
% Salient Translation Error Detection & 37.3 & \textbf{46.0} & 37.3 & 37.3 \\
% Snarks & 50.0 & \textbf{55.1} & 51.8 & 59.0 \\
% Sports Understanding & \textbf{56.0} & \textbf{56.0} & 48.3 & 53.3 \\
% Temporal Sequences & 16.7 & \textbf{26.7} & 18.7 & 21.3 \\
% \begin{tabular}[c]{@{}l@{}}Tracking Shuffled Objects$^\S$ \\ {\small ~~~~~~~~~~~~~\quad\quad\quad(five objects)}\end{tabular} & \textbf{12.0} & \textbf{12.0} & \textbf{12.0} & 12.0 \\
% \begin{tabular}[c]{@{}l@{}}Tracking Shuffled Objects$^\S$ \\ {\small ~~~~~~~~~~~~~\quad\quad\quad(seven objects)}\end{tabular} & 6.7 & 6.7 & \textbf{7.1} & 8.7 \\
% \begin{tabular}[c]{@{}l@{}}Tracking Shuffled Objects$^\S$ \\ {\small ~~~~~~~~~~~~~\quad\quad\quad(three objects)}\end{tabular} & 24.7 & \textbf{30.7} & 29.0 & 30.7 \\
% Web of Lies & \textbf{54.0} & \textbf{54.0} & 53.0 & 54.7 \\
% Word Sorting & \textbf{1.3} & 0.7 & 1.1 & 1.3 \\
% \midrule
% Average Performance per Task & 27.0 & \textbf{37.5} & 34.7 & 38.3 \\
% Average Consumed Tokens per Example & \textbf{111.6} & 597.8 & \textbf{111.6} & 111.6 \\
% \bottomrule
% \end{tabular}
% \end{table}
